Neurosymbolic Reinforcement Learning with Formally Verified Exploration

We present Revel, a partially neural reinforcement learning (RL) framework for provably safe exploration in continuous state and action spaces. A key challenge for provably safe deep RL is that repeatedly verifying neural networks within a learning loop is computationally infeasible. We address this challenge using two policy classes: a general, neurosymbolic class with approximate gradients and a more restricted class of symbolic policies that allows efficient verification. Our learning algorithm is a mirror descent over policies: in each iteration, it safely lifts a symbolic policy into the neurosymbolic space, performs safe gradient updates to the resulting policy, and projects the updated policy into the safe symbolic subset, all without requiring explicit verification of neural networks. Our empirical results show that Revel enforces safe exploration in many scenarios in which Constrained Policy Optimization does not, and that it can discover policies that outperform those learned through prior approaches to verified exploration.

==> implementation.tex <==
\section{Implementation}
We will now discuss one particular programmatic policy class, and see how we can instantiate the projection operation for this class. In order to facilitate verification, the class we use for our experiments consists of piecewise linear policies with a fixed bound on the number of cases. Let $f_1, \ldots, f_n$ be a set of linear functions and $P_1, \ldots, P_n$ be a partition of the state space such that $f$ applies the linear function $f_i$ to each state in $P_i$. Then for a programmatic policy $f$ we look for an invariant of the form $\phi = \phi_1 \vee \cdots \vee \phi_n$ where $\phi_i$ and $\phi_j$ are disjoint for each $i \neq j$. Then for each $i$, we require that $x \vdash \phi_i \implies f_i(x) \vdash \phi$ and $P_i \cap \states_0 \vdash \phi_i$. Finally, we require that $\phi$ does not include any unsafe states, i.e., for all $x \in \states_U$, $x \nvdash \phi$. Intuitively, we associate a condition $\phi_i$ with each partition $P_i$. Then whenever the current state satisfies one of these conditions, we require that applying the associated function gives us a state which still satisfies one condition (though it may be a different one). Then the disjunction of all of these conditions is an inductive invariant for $f$ as a whole. Moreover, we require that each $\phi_i$ covers the set of initial states which is in its associated partition to guarantee that the initial states of the system are safe.

In order to project a blended policy into this programmatic policy space, we take inspiration from MARS~\cite{Friedman91multivariateadaptive}, a well-known technique for fitting piecewise linear models to data. Specifically, we sample a number of partitions of the state space. Then for each partition, we fit a linear model to each set in the partition and measure the given Bregman divergence. The partition which yields the lowest divergence is taken as the new programmatic policy. However in order to guarantee that we can find an invariant for the new policy, we restrict the partitions we can choose and we modify the process for fitting each linear model. Our specific approach is presented in Algorithm~\ref{alg:project}



Algorithm~\ref{alg:project} starts by using the old programmatic policy $f$. It then samples a number of partitions which are \emph{consistent} with $f$ in the sense that if the set $p$ is in the partition $P$ then there exists $p'$ in the partition of $f$ such that $p \subseteq p'$. This restriction is useful in the next call to \Call{ImitateSafely}{}, which will be discussed below. \Call{ImitateSafely}{} returns a policy which imitates the neural network given the partition $P$. Finally, Algorithm~\ref{alg:project} simply keeps track of the best policy and returns it at the end.

% \begin{algorithm}
% \caption{Safely imitating a network using a given starting point and partition.}
% \label{alg:imitate}
% \begin{algorithmic}
% \Procedure{ImitateSafely}{$f, \phi, N, P$}
% \State $\pi \gets \varnothing$
% \For{$p \in P$}
%   \State $\psi \gets \phi|_p$
%   \State $f' \gets f$
%   \While{*}
%     \State $S \gets \Call{ComputeSafeRegion}{f', \psi}$
%     \State $f' \gets f' - \alpha \nabla_f' D(f', N)$
%     \State $f' \gets \textit{proj}_S(f')$
%   \EndWhile
%   \State $\pi \gets \pi \cup \{(p, f')\}$
% \EndFor
% \State \textbf{return} $\pi$
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

Algorithm~\ref{alg:imitate} describes how to imitate a neural network with a piecewise-linear controller when the partition is fixed. The complication here comes from the fact that we must choose a controller which is verifiable. In order to do this, we start with the controller $f$ which is known to be safe with the invariant $\phi$. Recall that $\phi$ is a disjunction of conditions, where each condition applies to one of the sets in the partition of $f$. Further, remember that we assumed $P$ was consistent with $f$. Then we'll let $\phi|_p$ for some $p \in P$ mean the disjunct of $\phi$ which is associated with the set $p'$ in the partition of $f$, such that $p \subseteq p'$.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec_background.tex <==
\section{Background: Mirror Descent and \propel}
\label{sec:background}

Notice that our policy representation includes two different kinds of policies: standard neural networks and shields. One kind admits gradient updates while the other places constraints on the policy to make it more easily verifiable. This setup is similar to that explored by \propel~\cite{propel}, a variant of mirror descent designed for training hybrid policies. \propel\ maintains a blended policy consisting of a linear combination of a neural network with a symbolic program. This policy is trained by alternating updates of the neural network with updates of the programmatic policy. The neural network can be trained using standard techniques, while the projection is done using a form of imitation learning.

While \propel\ is able to produce programmatic policies which are more interpretable and generalizable than deep neural networks, it does not lend itself to formal verification, particularly during training time. Thus, we are not able to directly apply \propel\ to our setting, but we use it as a basis to explore update-and-project approaches to the verified exploration problem.

==> sec_policies.tex <==
\section{Shielded Neural Policies}
\label{sec:policies}

In order to solve the safe reinforcement learning problem defined in Section~\ref{sec:Problem}, we need to choose a policy representation which allows for both optimization and verification. While neural networks have emerged as the de-facto standard for representing policies, they are difficult to verify due to their high-dimensionality and complex behavior. Thus, to make safe RL more tractable, we adopt a policy representation that  we refer to as \emph{shielded neural policies}:

\begin{definition}[Shielded neural policy]
A shielded neural policy (SNP) $\pi$ is a pair $(\mathcal{N}, \mathcal{F})$ where $\mathcal{N}$ is a neural network, and $\mathcal{F}$ is a (finite) set of \emph{guarded linear functions} of the form $(\phi_i, f_i)$ where $\phi_i$ is a boolean condition and $f_i$ is a linear function. We additionally require that $\states_0 \subseteq \bigcup_i \{x \in \states \mid \phi_i(x)\}$, i.e., each initial state satisfies at least one of the guards.
\end{definition}
Given an SNP  $(\mathcal{N}, \mathcal{F})$, we refer to  $\mathcal{F}$ as the \emph{shield} for $\mathcal{N}$, and we refer to any $(\phi_i, f_i) \in \mathcal{F}$ as a \emph{component} of the shield.

We also define a corresponding notion of \emph{trajectory} for shielded neural policies as follows:

\begin{definition}[SNP trajectory]
Given an SNP $\pi$ and starting state $s_0$ of MDP $(\mathcal{S}, \mathcal{A}, P, r, p_0, r, \gamma, t)$, a trajectory is a sequence $(s_0, a_0), \ldots, (s_t, a_t)$ such that:
\[
a_{i} = \left \{
\begin{array}{ll}
    \mathcal{N}(s_{i}) & \forall x \in \supp(P(s_i, \mathcal{N}(s_i))) : \exists j : \phi_j(x) \\
    f_j(s_i) & \phi_j(s_i) \\
    f_{k_{i - 1}} & \text{otherwise}
\end{array}
\right .
\]
(where $k_i$ is the index of the controller used at time step $i$) and $s_{i+1} \in \supp(P(s_i, a_i))$.

\end{definition}

We can now define what it means for a shielded neural policy to be \emph{safe}:

\begin{definition}[Safe SNP]
Let $M$ be an MDP, and let $\pi$ be a  shielded neural policy for $M$. We say that $\pi$ is a \emph{safe shielded neural policy}, if all trajectories $t$ of $\pi$ (starting from an initial state of $M$) are safe.
\end{definition}

To see why we choose SNPs as our policy representation, observe that the problem of verifying the safety of an SNP is much simpler than that of verifying the safety of a neural network. In particular, as shown in Algorithm??, verifying an SNP only requires verifying the safety of the shield but not the network itself.  In particular, since the SNP acts according to the shield whenever the neural network is in danger of  taking an unsafe action,  we do not need to verify the safety of the network. As long as each component of the shield can be individually proven safe, then the entire SNP is guaranteed to be safe.


\begin{algorithm}[!t]
\caption{Verifying a shielded neural policy.}
\label{alg:verif}
\begin{algorithmic}
\Procedure{VerifySNP}{$N, \mathcal{F}$}
  \For{$1 \le i \le n$}
    \State $S \gets \{s \in \states_0 \mid \phi_i(s)\}$
    \For{$1 \le j \le t$}
      \State $S \gets S \cup P^\#(S, \{f_i(s) \mid s \in S\})$
    \EndFor
    \If{$s \cap \states_U \neq \varnothing$}
      \State \textbf{return} false
    \EndIf
  \EndFor
  \State \textbf{return} true
\EndProcedure
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:verif} 

The following theorem states the soundness of {\sc VerifySNP} procedure from Algorithm~\ref{alg:snp}.
\begin{theorem}
Let $\pi$ be a shield neural network for $M$. Then, if {\sc VerifySNP}($\pi$) returns \emph{true}, then $\po$ is indeed a safe policy for $M$.
\end{theorem}


\begin{comment}

A shielded neural policy consists of a neural network along with another policy in a lower-dimensional space which can be efficiently verified. In our case, the lower-dimensional policy space consists of piece-wise linear functions with a bounded number of pieces. 


Intuitively, this representation allows for easy verification because each linear piece can be considered separately over the portion of the state space where it applies. Then in order to execute the shielded neural policy, we first attempt to use the network, and look ahead one time step to see if the resulting state is still within the region for which the piecewise linear function has been verified. If it is, then we can use the network. Otherwise, we fall back to the piecewise linear controller.

More formally, a \emph{shield} consists of a set of $n$ matrices $\{K_i\}_{i=1}^n$ and $n$ polytopes $\{P_i\}_{i=1}^n$ such that $\bigcup_i P_i$ includes each initial state of the system. For a given time horizon $t$, each matrix is safe over its associated polytope in the following sense: starting from any initial state $x_0 \in P_i$, we define a sequence of states $x_{i+1} = e(x_i, K_i x_i)$ where $e$ is the environment step function. That is, we repeatedly use the matrix $K_i$ to transform the current state into an action to apply. Then either $x_i$ is a safe state for each $1 \le i \le t$ or there exists some $i$ such that $x_i \in P_j$ for some $j$. In the first case, the safety result is straightforward because each state is already safe. In the second case, the trajectory under the given controller moves into the region covered by another controller. Then that controller is safe up to time horizon $t$ in turn, so the shield as a whole is still guaranteed to be safe.

\begin{algorithm}
\caption{Using a shielded neural policy.}
\label{alg:snp}
\begin{algorithmic}
\Procedure{ExecuteSNP}{$N, \{K_i\}_{i=1}^n, \{P_i\}_{i=1}^n, x_0, t$}
  \State $\ell \gets 0$
  \For{$1 \le \tau \le t$}
    \State $x' \gets e(x_{\tau-1}, N(x_{\tau-1}))$
    \If{$\exists j, x' \in P_j$}
      \State $x_\tau \gets x'$
    \ElsIf{$\exists j, x_{\tau-1} \in P_j$}
      \State $x_\tau \gets K_j x_{\tau-1}$
      \State $\ell \gets j$
    \Else
      \State $x_\tau \gets K_\ell x_{\tau-1}$
    \EndIf
  \EndFor
  \State \textbf{return} $\{x_0, \ldots, x_t\}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

Now a shielded neural policy consists of a neural network $N$ and a shield. Algorithm~\ref{alg:snp} describes how to evolve a system trajectory under a given shielded neural policy. The algorithm takes a network $N$, a shield defined by it's matrices $K_i$ and polytopes $P_i$, an initial state $x_0$ and a time horizon $t$. We first initialize a local variable $\ell$ which keeps track of which shield was last executed. For each time step, we first look ahead one step to determine whether we can use the neural network. If we can use the neural network, then we do. Otherwise, we must use one of the linear controllers from the shield. There are two possibilities: (1) the current system state is still in the polytope covered by some linear controller, or (2) the system state is no longer in the union of the shield's polytopes. In case (1), we just execute the linear controller whose polytope covers the current state. Note that case (2) can only happen after one of the linear controllers has been called at least once because if the system state were ever to leave the covered region under the network, then the shield would intervene. Therefore if we reach case (2), we know that $\ell$ points to the last executed shield. In this case we continue to use the last executed shield.


\begin{theorem}
For any neural network $N$ and shield $\{K_i\}_{i=1}^n$, $\{P_i\}_{i=1}^n$ which has been verified to a time horizon $t$, and for any initial state $x_0$, let $\{x_0, \ldots, x_t\} = \Call{ExecuteSNP}{N, \{K_i\}, \{P_i\}, x_0, t}$. Then $x_i$ is a safe state for each $0 \le i \le t$.
\end{theorem}
\begin{proof}
Prove this.
\end{proof}

\end{comment}

==> sec_shielded_training.tex <==
\section{Training Shielded Neural Policies}
\label{sec:training}

Training shielded neural policies involves two alternating phases, inspired by [cite Propel]. In one phase, we train the neural network component of the policy using a well-established technique (e.g., deep deterministic policy gradients). In the other phase, we update the shield component of the policy so that its behavior is more similar to the network.

The shield update can be viewed as a projection step, in which the (high-dimensional, complex) behavior of the neural network is projected onto a (low-dimensional, simpler) shield.
